Feature matching as improved transfer learning technique for wearable EEG

Objective: With the rapid rise of wearable sleep monitoring devices with non-conventional electrode configurations, there is a need for automated algorithms that can perform sleep staging on configurations with small amounts of labeled data. Transfer learning has the ability to adapt neural network weights from a source modality (e.g. standard electrode configuration) to a new target modality (e.g. non-conventional electrode configuration). Methods: We propose feature matching, a new transfer learning strategy as an alternative to the commonly used finetuning approach. This method consists of training a model with larger amounts of data from the source modality and few paired samples of source and target modality. For those paired samples, the model extracts features of the target modality, matching these to the features from the corresponding samples of the source modality. Results: We compare feature matching to finetuning for three different target domains, with two different neural network architectures, and with varying amounts of training data. Particularly on small cohorts (i.e. 2 - 5 labeled recordings in the non-conventional recording setting), feature matching systematically outperforms finetuning with mean relative differences in accuracy ranging from 0.4% to 4.7% for the different scenarios and datasets. Conclusion: Our findings suggest that feature matching outperforms finetuning as a transfer learning approach, especially in very low data regimes. Significance: As such, we conclude that feature matching is a promising new method for wearable sleep staging with novel devices.

==> oldintro.tex <==
In the field of deep domain adaptation, a branch of transfer learning, domain mapping and domain-invariant feature learning are common strategies to align source and target domain features onto each other \cite{Wilson2018}. Common approaches include domain-adversarial neural networks \cite{Ganin2015} and approaches using the maximum mean discrepancy (MMD) loss \cite{Tzeng2014DeepInvariance, Long2015LearningNetworks}. %Supervised domain adaptation techniques from the image processing field \cite{Hedegaard2020SupervisedProtocol, Wang2020DomainMatching, Motiian2017UnifiedGeneralization, Xu2019D-SNE:Embedding} use different approaches to align the feature spaces of two domains. However, to our knowledge, such supervised domain matching techniques have not been employed in EEG applications yet. \
\textcolor{red}{Unsupervised domain adaptation techniques have already been applied to EEG-based tasks in applications such as emotion recognition and motor imagery in brain-computer interfaces \cite{Hong2021DynamicClassification, Bao2021Two-LevelRecognition, Zhao2021DeepClassification, Chai2016UnsupervisedRecognition, Li2020DomainSimilarity}. %Nasiri2021}. 
These domain adaptation techniques have mainly focused on personalization, cross-session adaptation and domain mismatch between different datasets, with the same or very similar channels from both datasets. The application of these methods has therefore been limited to settings where %the source and target dataset are of the same modality and where 
differences between the source and target distribution are relatively small. In this work, we focus on transfer learning between different recording positions. The difference between the waveforms of the source domain and target domain in our use case is therefore much larger, explaining why unsupervised domain adaptation has not yet successfully been applied for this application, while the supervised finetuning technique has been proven to work well. We aim to combine strengths of both approaches in our new transfer learning technique.}

\textcolor{red}{Inspired by the supervised technique of finetuning on the one hand, and unsupervised domain adaptation techniques on the other hand, we propose a novel transfer learning technique (see Fig. \ref{fig:overview}) that aligns the feature space of a new EEG modality (the target domain) with that of a standard EEG modality (the source domain). The large difference between the source domain and target domain in our use case motivates the use of limited labeled data like in the finetuning approach. %, but we adopt a more flexible feature matching framework inspired from field of domain adaptation. 
Additionally, differently from existing domain adaptation techniques for EEG, we make use of a separate encoding network for the source modality and target modality, as the differences between both domains are too large to use a common encoder. Lastly, instead of using the MMD loss or an adversarial discriminator to match both domains, we facilitate domain matching on these signals with the use of a paired metric, the mean squared error (MSE). Although this is not the case in all applications, our use case allows using the MSE with paired target and source samples.
%In order to facilitate the process of domain matching on these signals, our method differs from other techniques in that it uses paired target and source samples.
%While in image applications, the goal is to align clouds of discrete points, EEG signals are continuous with less clear class boundaries. In order to facilitate the process of domain matching on these signals, our method differs from other techniques in that it uses paired target and source samples.
%propose a novel, improved transfer learning approach that allows sleep staging algorithms to be trained on standard modalities and adapt to new ones (see figure \ref{fig:overview}). 
%Instead of purely relying on label information like the finetuning method, our technique thus also exploits the correspondence between the source modality and target modality of the same sample. 
Indeed, labeled datasets with wearable EEG data always include simultaneous recordings of the standard and wearable EEG modalities, because the standard EEG is needed for manual labeling. Therefore, we can use the information in this correspondence to improve the sleep staging performance on small wearable EEG datasets.
%By using this additional information to improve the sleep staging performance,%
%Like domain adaptation techniques in image processing \cite{Hedegaard2020SupervisedProtocol, Wang2020DomainMatching, Motiian2017UnifiedGeneralization, Xu2019D-SNE:Embedding}, we align the source and target domains. 
We demonstrate that, by using this additional domain information, feature matching outperforms simple finetuning in sleep staging tasks on small, wearable EEG datasets. Moreover, we show that minimizing the MSE between paired samples leads to better results than using a non-paired metric such as the MMD, which matches two distributions onto each other without taking paired samples into account.}\
